Grounding Recursive Aggregates: Preliminary Report

Problem solving in Answer Set Programming consists of two steps, a first grounding phase, systematically replacing all variables by terms, and a second solving phase computing the stable models of the obtained ground program. An intricate part of both phases is the treatment of aggregates, which are popular language constructs that allow for expressing properties over sets. In this paper, we elaborate upon the treatment of aggregates during grounding in Gringo series 4. Consequently, our approach is applicable to grounding based on semi-naive database evaluation techniques. In particular, we provide a series of algorithms detailing the treatment of recursive aggregates and illustrate this by a running example.

==> extra/aggregates.tex <==
The Company Controls encoding has only one recursive aggregate occurrence.
The following example illustrates all of the different types of aggregate occurrences:%
\footnote{This is some syntactic graph problem to illustrate the different kind of aggregates.
  The graph is given by atoms over predicate~\Pred{v} for vertices and atoms over predicate~\Pred{e} for edges.
  The encoding marks a vertex as reached using predicate~\Pred{r} if 
  it has no incoming edges~(\ref{eq:aggregate:strat}),
  its predecessor is reached and the vertex itself has no outgoing edges~(\ref{eq:aggregate:strat-rec}), or
  at least three predecessors of the vertex are reached~(\ref{eq:aggregate:rec}).}
\begin{align}
  % reached if no incoming edges (stratified aggregate)
  \Pred{r}(Y) & \leftarrow \Pred{v}(Y) \wedge \Sum^+ \{ 1,X : \Pred{e}(X,Y) \} \leq 0 \label{eq:aggregate:strat}\\
  % reached if no outgoing edges (recursive grounding resulting in stratified aggregate)
  \Pred{r}(Y) & \leftarrow \Pred{r}(X) \wedge \Pred{e}(X,Y), \Sum^+ \{ 1,Z : \Pred{e}(Y,Z) \} \leq 0 \label{eq:aggregate:strat-rec}\\
  % reached if at least three incoming edges
  \Pred{r}(Y) & \leftarrow \Pred{v}(Y) \wedge \Sum^+ \{ 1,X : \Pred{r}(X), \Pred{e}(X,Y) \} \geq 3 \label{eq:aggregate:rec}
\end{align}
% rewriting of the above rules
%\begin{align*}
%  \Accu_1(Y,\Neutral)    & \leftarrow B_1^\dagger \wedge 0 \leq 0 &
%  \Aggr_1(Y)             & \leftarrow \Accu_1(Y,\_) \wedge \bot\\
%  \Accu_1(Y,\Tuple(1,X)) & \leftarrow B_1^\dagger \wedge \Pred{e}(X,Y) &
%  \Pred{r}(Y)            & \leftarrow B_1 \wedge \Aggr_1(Y)\\
%  \midrule
%  %---------------------------------------------------------------------%
%  \Accu_2(Y,\Neutral)    & \leftarrow B_2^\dagger \wedge 0 \leq 0 &
%  \Aggr_2(Y)             & \leftarrow \Accu_2(Y,\_) \wedge \bot\\
%  \Accu_2(Y,\Tuple(1,Z)) & \leftarrow B_2^\dagger \wedge \Pred{e}(Y,Z) &
%  \Pred{r}(Y) & \leftarrow B_2 \wedge \Aggr_2(Y)\\
%  \midrule
%  %---------------------------------------------------------------------%
%  \Accu_3(Y,\Neutral)    & \leftarrow B_3^\dagger \wedge 0 \geq 3 &
%  \Aggr_3(Y)             & \leftarrow \Accu_3(Y,\_) \wedge \bot\\
%  \Accu_3(Y,\Tuple(1,X)) & \leftarrow B_3^\dagger \wedge \Pred{r}(X) \wedge \Pred{e}(X,Y) &
%  \Pred{r}(Y) & \leftarrow B_2 \wedge \Aggr_3(Y)
%\end{align*}
\begin{tikzpicture}[
    node distance=5mm and 5mm,
    %every node/.style={font=\scriptsize\ttfamily},
    rule/.style={rectangle,minimum size=5mm,draw=black},
    posEdge/.style={->},
    negEdge/.style={->,dotted},
    compPN/.style={draw,dashdotted},
    compP/.style={draw,dashed}]

  \node (empty1) [rule] {\(\Accu_1(Y,\Neutral) \leftarrow B_1^\dagger \wedge 0 \leq 0\)};
  \node (accu1)  [rule,right=of empty1] {\(\Accu_1(Y,\Tuple(1,X)) \leftarrow B_1^\dagger \wedge \Pred{e}(X,Y)\)};
  \node (aggr1)  [rule,below=of empty1] {\(\Aggr_1(Y) \leftarrow \Accu_1(Y,\_) \wedge \bot\)};
  \node (rule1)  [rule,below=of aggr1] {\(\Pred{r}(Y) \leftarrow B_1 \wedge \Aggr_1(Y)\)};
  \node (empty3) [rule,at=(rule1 -| accu1)] {\(\Accu_3(Y,\Neutral) \leftarrow B_3^\dagger \wedge 0 \geq 3\)};

  \node (empty2) [rule,below=of rule1] {\(\Accu_2(Y,\Neutral) \leftarrow B_2^\dagger \wedge 0 \leq 0\)};
  \node (accu2)  [rule,below=of empty2] {\shortstack[l]{\(\Accu_2(Y,\Tuple(1,Z)) \leftarrow\)\\\(\qquad B_2^\dagger \wedge \Pred{e}(Y,Z)\phantom{\underline{r(X)}}\)}};
  \node (aggr2)  [rule,below=of accu2] {\(\Aggr_2(Y) \leftarrow \underline{\Accu_2(Y,\_)} \wedge \bot\)};
  \node (rule2)  [rule,below=of aggr2] {\(\Pred{r}(Y) \leftarrow B_2 \wedge \underline{\Aggr_2(Y)}\)};

  \node (accu3)  [rule,at=(accu2 -| empty3)] {\shortstack[l]{\(\Accu_3(Y,\Tuple(1,X)) \leftarrow\)\\\(\qquad B_3^\dagger \wedge \underline{\Pred{r}(X)} \wedge \Pred{e}(X,Y)\)}};
  \node (aggr3)  [rule,below=of accu3] {\(\Aggr_3(Y) \leftarrow \underline{\Accu_3(Y,\_)} \wedge \bot\)};
  \node (rule3)  [rule,below=of aggr3] {\(\Pred{r}(Y) \leftarrow B_2 \wedge \underline{\Aggr_3(Y)}\)};

  \coordinate (left) at ($(empty2.west)-(5mm,0)$);
  \coordinate (left2) at ($(empty2.west)-(3.25mm,0)$);
  \coordinate (right) at ($(empty3.east)+(3.25mm,0)$);
  \coordinate (center) at ($(empty2)!0.5!(empty3)$);
  \coordinate (top) at (rule1 -| center);
  \coordinate (bottom) at ($(rule3.south)-(0,3.25mm)$);
  \draw (rule1) -- (empty3)
        (top) |- (rule3)
        (top |- rule3) -- (rule2)
        (rule1) -| (center)
        (left2 |- accu2) -- (accu2)
        (rule3) -- (bottom) -| (left |- rule2)
        ;
  \draw[<->] (accu2) -- (accu3);
  \draw[posEdge] (accu1) |- (aggr1);
  \draw[posEdge] (top |- empty2) -- (empty2);
  \draw[posEdge] (aggr1) -- (rule1);
  \draw[posEdge] (empty1) -- (aggr1);
  \draw[posEdge] (rule1) -| (left) |- (rule2);
  \draw[posEdge] (empty2) -- (left2) |- (aggr2);
  \draw[posEdge] (empty3) -- (right) |- (aggr3);
  \draw[posEdge] (right |- accu3) -- (accu3);
  \draw[posEdge] (aggr2) -- (rule2);
  \draw[posEdge] (aggr3) -- (rule3);

  \fill (top |- rule3)   circle [radius=1pt]
        (top)            circle [radius=1pt]
        (top |- empty2)  circle [radius=1pt]
        (top|-accu2)     circle [radius=1pt]
        (left2 |- accu2) circle [radius=1pt]
        (right |- accu3) circle [radius=1pt]
        (left |- rule2)  circle [radius=1pt];
  \node [compPN,fit=(accu1)] {};
  \node [compPN,fit=(empty1)] {};
  \node [compPN,fit=(rule1)] {};
  \node [compPN,fit=(empty3)] {};
  \node [compPN,fit=(aggr1)] {};
  \node [compPN,fit=(empty2) (aggr3) (rule3)] {};
\end{tikzpicture}\\
where \(B_1 = \Pred{v}(Y)\), \(B_2 = \underline{\Pred{r}(X)} \wedge \Pred{e}(X,Y)\), and \(B_3 = \Pred{v}(Y)\).

The first aggregate is stratified and is only added to the set \ref{eq:aggregate:strat}
(for the component where \(\Aggr_1\) occurs in the body).
The rewriting of the three rules above has only one component involving recursive predicates,
which contains the (rewritten) rules for (\ref{eq:aggregate:strat-rec}) and (\ref{eq:aggregate:rec}).
Hence, the unique identifiers of the two aggregates are collected in \(\RecAggr\).
Because non of the aggregate elements of the aggregate in (\ref{eq:aggregate:strat-rec}) is recursive,
it is added to the set of stratified aggregates \StratAggr.



==> extra/nonlinear.tex <==
\subsection{Additional nonlinear Example that will probably not be included in the Paper}
To see this, consider the simple program\comment{this example could already be given in the introduction}
\begin{align}
  p(X,Z) & \leftarrow \DomNew(p(X,Y)) \wedge \DomAll(p(Y,Z))  \label{eq:trans:r1} \\
  p(X,Z) & \leftarrow \DomOld(p(X,Y)) \wedge \DomNew(p(Y,Z)). \label{eq:trans:r2}
\end{align}
Now assume we ground this program w.r.t.\ the initial set of atoms \(\{ p(1,2), p(2,3), p(3,4) \}\).
The grounding is depicted in the following table:
\begin{table}[H]
  \centering
\begin{tabular}{lllll}
  \toprule
  \(i\) & \(O_i\) (Old) & \(N_i\) (New) & \(A_i\) (All) & Rules\(_i\)\\
  \midrule
  1 & \(\emptyset\) & \( N_0\)                 & \(\emptyset \cup N_1\) & \(p(1,3) \leftarrow \DomNew(p(1,2)) \wedge \DomAll(p(2,3)) \) \\
    &               &                          &                        & \(p(2,4) \leftarrow \DomNew(p(2,3)) \wedge \DomAll(p(3,4)) \) \\
  2 & \(A_1\)       & \(\{ p(1,3), p(2,4) \}\) & \( A_1 \cup N_2 \)     & \(p(1,4) \leftarrow \DomNew(p(1,3)) \wedge \DomAll(p(3,4)) \) \\
    &               &                          &                        & \(p(1,4) \leftarrow \DomOld(p(1,2)) \wedge \DomNew(p(2,4)) \) \\
  3 & \(A_2\)       & \(\{ p(1,4) \}\)         & \( A_2 \cup N_3 \) \\
  \bottomrule
\end{tabular}
\end{table}
In Step 1 the domains \(O_1\), \(N_1\), and \(A_1\) of predicates \(\DomOld/1\), \(\DomNew/1\), and \(\DomAll/1\) are initialized w.r.t.\ the initial set of atoms.
Only Rule (\ref{eq:trans:r1}) contributes ground instances because the domain \(O_1\) for \(\DomOld/1\) is still empty,
which blocks Rule~(\ref{eq:trans:r2}).
In the next step both rules (\ref{eq:trans:r1}) and (\ref{eq:trans:r2}) contribute (different) instances.
In fact, each rule instance in each step contains at least one new positive body atom and no two equal instances are generated by the same non-ground rule.
The grounding stops in Step 3 because no new rules are generated.

Note that the algorithm reifies all positive atoms with \(\DomNew/1\) if there are no recursive predicates (Line \ref{fun:prepare:nonrec}).
Here the idea is that such a component can be grounded in one iteration;
only the initial set of atoms is used for instantiation.




==> relwork.tex <==
\section{Related Work}

\tbf


